Active Property Testing

One of the motivations for property testing of boolean functions is the idea that testing can serve as a preprocessing step before learning. However, in most machine learning applications, it is not possible to request for labels of fictitious examples constructed by the algorithm. Instead, the dominant query paradigm in applied machine learning, called active learning, is one where the algorithm may query for labels, but only on points in a given polynomial-sized (unlabeled) sample, drawn from some underlying distribution D. In this work, we bring this well-studied model in learning to the domain of testing. We show that for a number of important properties, testing can still yield substantial benefits in this setting. This includes testing unions of intervals, testing linear separators, and testing various assumptions used in semi-supervised learning. In addition to these specific results, we also develop a general notion of the testing dimension of a given property with respect to a given distribution. We show this dimension characterizes (up to constant factors) the intrinsic number of label requests needed to test that property. We develop such notions for both the active and passive testing models. We then use these dimensions to prove a number of lower bounds, including for linear separators and the class of dictator functions. Our results show that testing can be a powerful tool in realistic models for learning, and further that active testing exhibits an interesting and rich structure. Our work in addition brings together tools from a range of areas including U-statistics, noise-sensitivity, self-correction, and spectral analysis of random matrices, and develops new tools that may be of independent interest.

==> cluster-tester.tex <==
\newcommand{\err}{err}

A common condition assumed in semi-supervised learning is that data
satisfies the ``cluster assumption'' that points in the same cluster
tend to have the same label\cite{ssl:book06}.\footnote{In this we assume that the
problem of actually clustering the data, and what it means for data to
be in a cluster, has already been addressed by some existing
clustering algorithm.}  In this section we provide an algorithm
for testing this assumption, which also
serves as an important subroutine in the margin-testing algorithm in
Section \ref{sec:margin}.  Formally, the problem we consider here is
the following.
\begin{itemize}
\setlength{\itemsep}{1pt}
\setlength{\parskip}{0pt}

\item There are $N$ bins (``clusters'') $1,2,\ldots,N$.

\item There is an unknown probability distribution $D$ over examples, which
  together with the target function $f$, induces a distribution over pairs
  $(i,\ell)$, where $i \in \{1,\ldots,N\}$ and $\ell \in \{0,1\}$.
	Specifically, let $p_{i0} =\Pr((i,0))$ and $p_{i1} = \Pr((i,1))$.

\item Let $\err(f) = \sum_i \min(p_{i0},p_{i1})$.  The function $f$
satisfies the cluster assumption ($f \in \calP)$ if $\err(f)=0$.  The
function $f$ and is $\epsilon$-far from satisfying the assumption if
$\err(f) \geq \epsilon$, because
this is the minimum probability mass of points that would need to have
their labels flipped in order to make each cluster pure.
\end{itemize}
Note that {\em learning} property $\calP$ (either active or passive)
requires $\Omega(N)$ labeled examples.  Additionally, for
passive testing, there exist distributions $D$ that would require
$\Omega(\sqrt{N}/\epsilon)$ labeled examples: in
particular suppose bin 1 has $1 - O(\epsilon)$
probability mass (and is pure) and the others equally share the
remaining $O(\epsilon)$ probability mass and either
are each pure but random ($f \in \calP$) or are
each 50/50 ($f$ is $\epsilon$-far from $\calP$).   Distinguishing
these cases requires seeing at least two points in the same bin $i
\neq 1$, yielding the
$\Omega(\sqrt{N}/\epsilon)$ bound.   However, with active testing we
can do much better.

\begin{theorem}
We can use Active Testing to test the cluster assumption with
$O(1/\epsilon)$ labeled examples and $O(N/\epsilon)$ unlabeled examples.
\end{theorem}
\begin{proof}
The tester is as follows.
\begin{enumerate}
\setlength{\itemsep}{1pt}
\setlength{\parskip}{0pt}
\item Draw a set $U$ of $O(N/\epsilon)$
unlabeled examples.
\item Repeat $4/\epsilon$ times: \\
Choose a random $x \in U$.
If $x$ is not the only example in its bin, choose
random $y \neq x$ in $x$'s bin, request the labels of $x$ and $y$, and
reject if $f(x) \neq f(y)$.
\item If $f$ was not rejected above, then accept.
\end{enumerate}
Clearly, if $f \in \calP$ the above procedure will accept, so suppose
$f$ is $\epsilon$-far from $\calP$.  Now, viewing $\calP$ as a
hypothesis class of $2^N$ functions, and viewing $\err(f)$ as the
error rate of the best $h \in \calP$ with respect to $f$, by standard
sample complexity bounds~\cite{KV:book94,VC,Vapnik:book98} we have that $|U|$ is sufficient such that with high
probability, $f$ is at least $\epsilon/2$-far from $\calP$ with
respect to the uniform distribution over $U$.  Assume this indeed is
the case.  This means that on each round of Step (2), $x$ is in the
minority class in its bin with probability $\geq \epsilon/2$.
Therefore, with probability $\geq \epsilon/4$, $y$ will have a
different label than $x$.  So, there is at least an $\epsilon/4$
chance that each round will reject $f$.
\end{proof}


==> margin-proofs.tex <==
\newtheorem*{thmmargin}{Theorem~\ref{thm:margin}}
\begin{thmmargin}[Restated]
For any $\gamma$, $\gamma' = \gamma(1-1/c)$ for constant $c>1$, for
data in the unit ball in $R^d$ for constant $d$, we can
distinguish the case that $D_f$ has margin $\gamma$ from the case that
$D_f$ is $\epsilon$-far from margin $\gamma'$ using Active Testing
with $O(1/(\gamma^{2d}\epsilon^{2}))$ unlabeled examples and
$O(1/\epsilon)$ label requests.
\end{thmmargin}

\newcommand{\witness}{E_{witness}}
\begin{proof}
First, partition the input space $X$ (the unit ball in $R^d$) into
regions $R_1, R_2, \ldots, R_N$ of diameter at most $\gamma/(2c)$.  By
a standard volume 
argument, this can be done using $N = O(1/\gamma^d)$ regions
(absorbing ``$c$'' into the $O()$).  Next, we run the cluster-property
tester on these $N$ regions, with distance parameter $\epsilon/4$.
Clearly, if the cluster-tester rejects, then we can reject as well.
Thus, we may assume below that the total impurity within individual
regions is at most $\epsilon/4$.

Now, consider the following weighted graph $G_\gamma$. We have $N$
vertices, one for each of the $N$ regions.  We have an edge $(i,j)$
between regions $R_i$ and $R_j$ if diam$(R_i \cup R_j) < \gamma$.  We
define the {\em weight} $w(i,j)$ of this edge to be
$\min(D[R_i],D[R_j])$ where $D[R]$ is the probability mass in $R$
under distribution $D$.  Notice that if there is no edge between
region $R_i$ and $R_j$, then by the triangle inequality every point in
$R_i$ must be at distance at least $\gamma'$ from every point in
$R_j$.  Also, note that each vertex has degree $O(c^d) = O(1)$, so the
total weight over all edges is $O(1)$.  Finally, note that while
algorithmically we do not know the edge weights precisely, we can
estimate all edge weights to $\pm \epsilon/(4M)$, where $M=O(N)$ is the
total number of edges, using the unlabeled sample size bounds given in
the Theorem statement.  Let $\tilde{w}(i,j)$ denote the estimated
weight of edge $(i,j)$.

Let $\witness$ be the set of edges $(i,j)$ such that one endpoint is
majority positive and one is majority negative.  Note that if $D_f$
satisfies the $\gamma$-margin property, then every edge in $\witness$
has weight 0. On the other hand, if $D_f$ is $\epsilon$-far from the
$\gamma'$-margin property, then the total weight of edges in
$\witness$ is at least $3\epsilon/4$.  The reason is that otherwise one
could convert $D_f$ to $D'_f$ satisfying the margin condition by
zeroing out the probability mass in the lightest endpoint of every
edge $(i,j) \in \witness$, and then for each vertex, zeroing out the
probability mass of points in the minority label of that vertex.
(Then, renormalize to have total probability 1.)  The first step
moves distance at most $3\epsilon/4$ and the second step moves
distance at most $\epsilon/4$ by our assumption of success of the
cluster-tester.  Finally, if the true total weight of edges in
$\witness$ is at least $3\epsilon/4$ then the sum of their estimated
weights $\tilde{w}(i,j)$ is at least $\epsilon/2$.
This implies we can perform our test as follows.  For $O(1/\epsilon)$
steps, do: 
\begin{enumerate}
\item Choose an edge $(i,j)$ with probability proportional to $\tilde{w}(i,j)$.
\item Request the label for a random $x \in R_i$ and $y\in R_j$.
If the two labels disagree, then reject.
\end{enumerate}
If $D_f$ is $\epsilon$-far from the $\gamma'$-margin property, then
each step has probability $\tilde{w}(\witness)/\tilde{w}(E) = O(\epsilon)$ of
choosing a witness edge, and conditioned on choosing a witness edge
has probability at least $1/2$ of detecting a violation.  Thus,
overall, we can test using $O(1/\epsilon)$ labeled examples and 
$O(1/(\gamma^{2d}\epsilon^2))$ unlabeled examples.
\end{proof}


\medskip
\noindent
{\bf On the necessity of slack in testing the margin assumption:}
Consider an instance space $\X = [0,1]^2$ and two distributions over
labeled examples $D_1$ and $D_2$.  Distribution $D_1$ has probability
mass $1/2^{n+1}$ on positive examples at location $(0, i/2^n)$ and
negative examples at $(\gamma', i/2^n)$ for each $i=1,2,\ldots, 2^n$,
for $\gamma' = \gamma(1 - 1/2^{2n})$.  Notice that $D_1$ is $1/2$-far
from the $\gamma$-margin property because there is a matching between
points in the support of $D_1|_{f=1}$ and points in the support of
$D_1|_{f=0}$ where the matched points have distance less than
$\gamma$.  On the other hand, for each $i=1,2,\ldots,2^n$,
distribution $D_2$ has probability mass $1/2^n$ at either a positive
point $(0, i/2^n)$ {\em or} a negative point $(\gamma', i/2^n)$,
chosen at random, but zero probability mass at the other location.
Distribution $D_2$ satisfies the $\gamma$-margin property, and yet
$D_1$ and $D_2$ cannot be distinguished using a polynomial number of
unlabeled examples.


==> margin-tester.tex <==
We now consider the property of a function having a large (or at least
noticeable) margin with respect to the underlying distribution: that
is, the distribution $D$ and target $f$ are such that any point in the
support of $D|_{f=1}$ is at distance $\gamma$ or more from any point
in the support of $D|_{f=0}$.  This is a common property assumed in
graph-based and nearest-neighbor-style semi-supervised learning
algorithms \cite{ssl:book06}.  Note that we are not additionally
requiring the target to be a linear separator or have any special
functional form.  For scaling, we assume that points lie in the unit
ball in $R^d$, where we view $d$ as constant and $1/\gamma$ as our
asymptotic parameter.\footnote{Alternatively points could lie in a
$d$-dimensional manifold in some higher-dimensional ambient space,
where the property is defined with respect to the manifold, and we
have sufficient unlabeled data to ``unroll'' the manifold using
existing methods \cite{ssl:book06,LLE,ISOMAP}.}  
Since we are not assuming any specific
functional form for the target, the number of labeled examples needed
for {\em learning} could be as large as $\Omega(1/\gamma^d)$
by having a distribution with support over $\Omega(1/\gamma^d)$ points
that are all at distance $\gamma$ from each other (and therefore can
be labeled arbitrarily).
%%, with points weighted as in the usual VC-dimension lower-bound.  
Furthermore, passive testing would require
$\Omega(1/\gamma^{d/2})$ samples as this specific case encodes the
cluster-assumption setting with $N =
\Omega(1/\gamma^d)$ buckets.  We will be able to perform active
testing using only $O(1/\epsilon)$ label requests.

First, one distinction between this and other properties we have
been discussing is that it is a property of the {\em relation} between the
target function $f$ and the distribution $D$; i.e., of the combined
distribution $D_f = (D,f)$ over labeled examples.  As a result, 
the natural notion of {\em distance} to this property is in
terms of the variation distance of $D_f$ to the closest $D_*$
satisfying the property.\footnote{As a simple example
illustrating the issue, consider $X = [0,1]$, a target $f$ that is
negative on $[0,1/2)$ and positive on $[1/2,1]$, and a distribution $D$
that is uniform but where the region $[1/2,1/2+\gamma]$ is
downweighted to have total probability mass only $1/2^n$.  Such a
$D_f$ is $1/2^n$-close to the property under variation distance, but
would be nearly $1/2$-far from the property if the 
only operation allowed were to change the function $f$.} 
Second, we will have to also allow some amount of slack on the
$\gamma$ parameter as well.  Specifically, our tester will distinguish
the case that $D_f$ indeed has margin $\gamma$ from the
case that the $D_f$ is $\epsilon$-far from having margin $\gamma'$
where $\gamma' = \gamma(1-1/c)$ for some constant $c>1$; e.g., think
of $\gamma' = \gamma/2$.  This slack can also be seen to be necessary
--- see Appendix \ref{app:margin-proofs}.
We now show the following.

\begin{theorem}
For any $\gamma$, $\gamma' = \gamma(1-1/c)$ for constant $c>1$, for
data in the unit ball in $R^d$ for constant $d$, we can
distinguish the case that $D_f$ has margin $\gamma$ from the case that
$D_f$ is $\epsilon$-far from margin $\gamma'$ using Active Testing
with $O(1/(\gamma^{2d}\epsilon^{2}))$ unlabeled examples and
$O(1/\epsilon)$ label requests.
\end{theorem}

\newcommand{\witness}{E_{witness}}
\begin{proof}
First, partition the input space $X$ (the unit ball in $R^d$) into
regions $R_1, R_2, \ldots, R_N$ of diameter at most $\gamma/(2c)$.  By
a standard volume 
argument, this can be done using $N = O(1/\gamma^d)$ regions
(absorbing ``$c$'' into the $O()$).  Next, we run the cluster-property
tester on these $N$ regions, with distance parameter $\epsilon/4$.
Clearly, if the cluster-tester rejects, then we can reject as well.
Thus, we may assume below that the total impurity within individual
regions is at most $\epsilon/4$.

Now, consider the following weighted graph $G_\gamma$. We have $N$
vertices, one for each of the $N$ regions.  We have an edge $(i,j)$
between regions $R_i$ and $R_j$ if diam$(R_i \cup R_j) < \gamma$.  We
define the {\em weight} $w(i,j)$ of this edge to be
$\min(D[R_i],D[R_j])$ where $D[R]$ is the probability mass in $R$
under distribution $D$.  Notice that if there is no edge between
region $R_i$ and $R_j$, then by the triangle inequality every point in
$R_i$ must be at distance at least $\gamma'$ from every point in
$R_j$.  Also, note that each vertex has degree $O(c^d) = O(1)$, so the
total weight over all edges is $O(1)$.  Finally, note that while
algorithmically we do not know the edge weights precisely, we can
estimate all edge weights to $\pm \epsilon/(4M)$, where $M=O(N)$ is the
total number of edges, using the unlabeled sample size bounds given in
the Theorem statement.  Let $\tilde{w}(i,j)$ denote the estimated
weight of edge $(i,j)$.

Let $\witness$ be the set of edges $(i,j)$ such that one endpoint is
majority positive and one is majority negative.  Note that if $D_f$
satisfies the $\gamma$-margin property, then every edge in $\witness$
has weight 0. On the other hand, if $D_f$ is $\epsilon$-far from the
$\gamma'$-margin property, then the total weight of edges in
$\witness$ is at least $3\epsilon/4$.  The reason is that otherwise one
could convert $D_f$ to $D'_f$ satisfying the margin condition by
zeroing out the probability mass in the lightest endpoint of every
edge $(i,j) \in \witness$, and then for each vertex, zeroing out the
probability mass of points in the minority label of that vertex.
(Then, renormalize to have total probability 1.)  The first step
moves distance at most $3\epsilon/4$ and the second step moves
distance at most $\epsilon/4$ by our assumption of success of the
cluster-tester.  Finally, if the true total weight of edges in
$\witness$ is at least $3\epsilon/4$ then the sum of their estimated
weights $\tilde{w}(i,j)$ is at least $\epsilon/2$.
This implies we can perform our test as follows.  For $O(1/\epsilon)$
steps, do: 
\begin{enumerate}
\item Choose an edge $(i,j)$ with probability proportional to $\tilde{w}(i,j)$.
\item Request the label for a random $x \in R_i$ and $y\in R_j$.
If the two labels disagree, then reject.
\end{enumerate}
If $D_f$ is $\epsilon$-far from the $\gamma'$-margin property, then
each step has probability $\tilde{w}(\witness)/\tilde{w}(E) = O(\epsilon)$ of
choosing a witness edge, and conditioned on choosing a witness edge
has probability at least $1/2$ of detecting a violation.  Thus,
overall, we can test using $O(1/\epsilon)$ labeled examples and 
$O(1/(\gamma^{2d}\epsilon^2))$ unlabeled examples.
\end{proof}



==> prelims.tex <==
\newcommand{\calQ}{\mathcal{Q}}

%%We introduce the basic tools that we will use in our proofs in this section.
%%All the proofs for the results presented in this section are deferred to
%%Appendix~\ref{app:prelims}.

The lower bounds on the query complexity for testing LTFs and dictators 
use a slight extension of a well-known lemma in property testing.  The proof of this lemma is deferred to Appendix~\ref{app:prelims}.

\enote{Todo: Update notation; simplify.}
\begin{lemma}
\label{lem:ptlb}
Let $D_1$ and $D_2$ be two distributions on functions $\R \to \R$.  Fix $\calQ \subseteq \R$ to be a set of allowable queries.  For a set $Q \in \calQ^q$ of $q$ queries, let $f_{1|Q}, f_{2|Q} : \R^q \to \R$ denote the pdfs of the distributions of the value of $g(Q)$ when $g \sim D_1, D_2$, respectively.  Suppose that for any set $Q \in \calQ^q$, there is a set $E_Q \subseteq \R^q$ such that the pdfs $f_{1|Q}$ and $f_{2|Q}$ satisfy
$$
f_{1|Q}(x) < \tfrac65 f_{2|Q}(x)
$$
for every $x \in \R_Q \setminus E_Q$ and such that
$$
\int_{E_Q} f_{1|Q}(x)\d x \le \tfrac15 2^{-q}.
$$
Then no algorithm that making at most $q$ queries from $\calQ$ can distinguish between  functions drawn from $D_1$ and functions drawn from $D_2$ with probability at least $\frac23$.
\end{lemma}


